Fine granularity access in interactive compression of 360-degree images based on rate-adaptive channel codes

In this paper, we propose a new interactive compression scheme for omnidirectional images. This requires two characteristics: efficient compression of data, to lower the storage cost, and random access ability to extract part of the compressed stream requested by the user (for reducing the transmission rate). For efficient compression, data needs to be predicted by a series of references that have been pre-defined and compressed. This contrasts with the spirit of random accessibility. We propose a solution for this problem based on incremental codes implemented by rate-adaptive channel codes. This scheme encodes the image while adapting to any user request and leads to an efficient coding that is flexible in extracting data depending on the available information at the decoder. Therefore, only the information that is needed to be displayed at the user's side is transmitted during the user's request, as if the request was already known at the encoder. The experimental results demonstrate that our coder obtains a better transmission rate than the state-of-the-art tile-based methods at a small cost in storage. Moreover, the transmission rate grows gradually with the size of the request and avoids a staircase effect, which shows the perfect suitability of our coder for interactive transmission.

==> acro_list.tex <==
%\acrodef{ldpc}[LDPC]{Low-Density Parity-Check}
%\acrodef{bp}[BP]{Belief Propagation}
%\acrodef{ic}[IC]{Interactive Compression/Coding}
%\acrodef{sw}[SW]{Slepian‐Wolf}
%\acrodef{bsc}[BSC]{Binary Symmetric Channel}
\acrodef{si}[SI]{Side Information}
%\acrodef{vn}[VN]{Variable Node}
%\acrodef{cn}[CN]{Check Node}
%\acrodef{llr}[LLR]{Log-likelihood ratio}
%\acrodef{de}[DE]{Density Evolution}
%\acrodef{biawgn}[BIAWGN]{binary input additive white Gaussian noise}
%\acrodef{exit}[EXIT]{Extrinsic Information Transfer Chart}
%\acrodef{kl}[KL]{Kullback–Leibler}

\acrodef{hmd}[HMD]{Head-Mounted Display}
\acrodef{ra_ldpc}[RA-LDPC]{Rate-Adaptive Low-Density Parity-Check}
\acrodef{dsc}{DSC}{Distributed Source Coding}
\acrodef{vvc}{VVC}{Versatile Video Coding}
\acrodef{cabac}{CABAC}{Context-based adaptive binary arithmetic coding}


==> algorithm_decoding_order.tex <==
\begin{figure}[h!]
\caption{Algorithm for decoding order when $m(\Gamma)$ is equirectangular projection. Comments are shown in \textit{italic} between /* and */.}\label{alg:decoding_order}
\begin{algorithmic}[1]
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\REQUIRE ~~\\
$\mathcal{J}(\theta)$: set of requested blocks \\
$\mathcal{A}$: set of access blocks \\
\ENSURE  permutation $\tau\big(\mathcal{J}(\theta)\big)$
\\ \textit{Initialization}: \\
$\mathcal{B} \leftarrow \mathcal{J}(\theta)$ \\
$i \leftarrow 0$

\STATE \textbf{Find} $k \in \mathcal{A}$ s.t. $k \in \mathcal{B}$
\STATE recursive\_processing\_neighbor$(k)$ % recursive\_processing\_neighbor

\RETURN $\tau\big(\mathcal{J}(\theta)\big)$
\end{algorithmic}

\quad

\begin{algorithmic}[1]
\renewcommand{\algorithmicensure}{\textbf{Function}}
\ENSURE recursive\_processing\_neighbor$(k)$:
\\ $pos: k \mapsto (x,y)$, converts block $k$ index to position in $m(\Gamma)$ \\
$n_{row}$: number of blocks per row in $m(\Gamma)$ \\
$n_{col}\ $: number of blocks per col in $m(\Gamma)$ \\
/* \textit{$dx, dy$ give the priority to process the horizontal neighbors first} */ \\
%\[
%\left.
%\begin{array}{ll}
%dx = [1,-1, 0, 0] \\
%dy = [0, 0, -1, 1]
%\end{array}
%\right\}
%\begin{array}{ll}
%
%\textit{/*(dx[0],dy[0]): \text{right block}} \\
%\textit{(dx[1],dy[1]): \text{left block}}  \\
%\textit{(dx[2],dy[2]): \text{upper block}} \\
%\textit{(dx[3],dy[3]): \text{lower block}*/}
%\end{array}
%\] \\
$dx = [1,-1, 0, 0]$ \\
$dy = [0, 0, -1, 1]$ \\
\quad
\STATE $\tau(k) \leftarrow i$ 
\STATE $ \mathcal{B} \leftarrow \mathcal{B} \setminus \{k\}$ /* \textit{remove $k$ from set $\mathcal{B}$} */
\IF { $\mathcal{B} = \emptyset$ }
\RETURN
\ENDIF
\STATE $ i \leftarrow i+1$
\STATE $(x,y) \leftarrow pos(k)$
\FOR{$j=0$ \TO $4$ }
\STATE $x_{neighbor} \leftarrow x + dx[j]$
\\ /* \textit{to enable  circular traversing for 360 video in x direction:} */
\STATE $x_{neighbor} \leftarrow x_{neighbor} \mod  n_{row}$ 
\STATE $y_{neighbor} \leftarrow y + dy[j]$
\IF {$y_{neighbor} \geq n_{col}$ or $y < 0$}
\STATE continue
\ENDIF
\STATE $k \leftarrow pos^{-1}(x_{neighbor}, y_{neighbor})$
\IF {$k \in \mathcal{B}$}
\STATE recursive\_processing\_neighbor$(k)$  /* \textit{recursive call} */
\ENDIF
\ENDFOR
\RETURN
\end{algorithmic}
\end{figure}

==> figures/S-R-D_curves.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,0.00000,0.10345}%
\definecolor{mycolor2}{rgb}{0.00000,0.00000,0.17241}%
\definecolor{mycolor3}{rgb}{1.00000,0.13793,0.75862}%
\definecolor{mycolor4}{rgb}{0.00000,0.37931,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=0.951\figurewidth,
height=\figureheight,
at={(0\figurewidth,0\figureheight)},
scale only axis,
xmin=40000,
xmax=140000,
tick align=outside,
xlabel style={font=\color{white!15!black}},
xlabel={${E}_{\theta}(R_\theta)$ (in bits)},
ymin=0,
ymax=1200000000,
ylabel style={font=\color{white!15!black}},
ylabel={$S$ (in bits)},
zmin=32,
zmax=48,
zlabel style={font=\color{white!15!black}},
zlabel={PSNR},
view={-66}{22},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
axis z line*=left,
xmajorgrids,
xminorgrids,
ymajorgrids,
yminorgrids,
zmajorgrids,
zminorgrids,
legend style={at={(0.334,0.433)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot3 [color=blue, mark=o, mark options={solid, blue}]
 table[row sep=crcr] {%
76567.278	83947256	47.5618597437672\\
69033.3946666667	76378304	44.6877098704151\\
64120.6086666667	71483192	41.729562460142\\
60650.2793333333	68062360	38.579951036718\\
58503.6613333333	65977528	35.5043519962588\\
56989.9686666667	64522368	32.405671786699\\
};
 \addlegendentry{Method A}

\addplot3 [color=mycolor1, mark=x, mark options={solid, mycolor1}]
 table[row sep=crcr] {%
90000.4933333333	83918000	47.5580581844253\\
81209.444	76344080	44.6884425214712\\
75475.4093333333	71443040	41.7214259789727\\
71436.1386666667	68022072	38.566560206353\\
68946.228	65940184	35.5009797833033\\
67195.352	64490352	32.3902525614234\\
};
 \addlegendentry{Method B}

\addplot3 [color=mycolor2, mark=square, mark options={solid, mycolor2}]
 table[row sep=crcr] {%
139816.706666667	83890024	47.5537920703021\\
127196.293333333	76317776	44.6822926186668\\
119017.253333333	71410352	41.7118209524827\\
113309.36	67985616	38.5589646901437\\
109853.08	65911848	35.4830437954466\\
107435.253333333	64461152	32.3570967522696\\
};
 \addlegendentry{Method C}

\addplot3 [color=mycolor3, mark=triangle, mark options={solid, rotate=180, mycolor3}]
 table[row sep=crcr] {%
63466.8973333333	1008023648	47.8114223580016\\
57258.1273333333	918230328	44.9661493484562\\
53176.4826666667	859374752	42.0706283427514\\
50265.576	817793040	38.9802292167046\\
48443.266	791926992	36.0099337718757\\
47116.1033333333	773296216	32.9791215406246\\
};
 \addlegendentry{Method D}

\addplot3 [color=mycolor4, mark=star, mark options={solid, mycolor4}]
 table[row sep=crcr] {%
125194.156916667	173044524	47.8114223580016\\
112786.708416667	158074404	44.9661493484562\\
104642.481416667	148224532	42.0706283427514\\
98841.3904166667	141105230	38.9802292167046\\
95211.0194166667	136622614	36.0099337718757\\
92584.0525833333	133249870	32.9791215406246\\
};
 \addlegendentry{Method E}

\end{axis}
\end{tikzpicture}%

==> sec_05.tex <==
% !TeX root = bare_jrnl.tex
%

\section{Evaluation Framework} \label{sec:evaluation_framework}
%Introducing this new type of interactive coding highlights the importance of presenting a new type of evaluation. Existing methods (see \cref{subsec:state_of_the_art}) scarify storage to have better transmission rate and redundant information between different representations is not taken into account during evaluation. Here, thanks to rate-adaptive codes and the proposed contributions we can avoid storing redundant data and at the same time having one stored stream per ICU. Therefore, storage is also an important element that must be considered during evaluation. More precisely, according to \eqref{eq:storage}, \eqref{eq:transmission_rate} and \eqref{eq:distortion} introduced in \cref{sec:problem_formulation} the triple of storage, transmission and distortion on the viewport should be considered all together as 3D data. 

To the authors' knownledge, there is no unified framework to evaluate interactive compression schemes, \emph{e.g.,} by differentiating between storage and transmission costs. In \cite{7328056} a framework is proposed to evaluate between different sphere-to-plane projection methods and since the whole content is sent to the user, classical rate-distortion (RD) curves are used for the evaluation. They also showed that the Peak Signal-to-Noise Ratio (PSNR) of \cref{eq:distortion} can be approximated by the weighted spherical PSNR. In \cite{7823595}, a rate allocation strategy is proposed to lower the transmission rate and therefore only $R_\theta$ is considered in the evaluation instead of RD curves. In \cite{8296518}, the sum of storage cost and RD curves are in the evaluation, but the trade-off between $S$ and $D_\theta$ is not taken into account.

In this section, we propose a framework to consider jointly storage, transmission rate and distortion. Therefore, contrary to conventional 2D image/video evaluation methodologies where 2D RD curves are used for comparison, here different methods must be compared in 3D with Storage-Rate-Distortion (S-R-D) values. It is worth noting that since the only free parameter in these schemes is the Quantization Parameter (QP) of the encoder, the S-R-D values generate 3D curves in the space. Examples of such curves are shown in \cref{fig:s-r-d_curve}. As it can be seen, performing a quantitative comparison between 3D curves is a difficult task especially because curves have different domain. We propose 3 ways to compare methods based on the constraints imposed by the system.

\begin{figure}[htb]
    \centering
    \fontsize{8pt}{8pt}\selectfont
\setlength\figurewidth{0.7\linewidth}
\setlength\figureheight{0.5\linewidth}
\input{./figures/S-R-D_curves.tex}
    \caption{Examples of S-R-D curves.}
	\label{fig:s-r-d_curve}
\end{figure}


\subsection{Average storage and transmission rate saving}
{\color{blue}Bjontegaard-Delta (BD) rate \cite{bjontegaard2001calculation} is a commonly used metric as it performs a fair comparison between two coding methods.
More precisely, a common PSNR range is determined and the average bitrate reduction/increase is computed for this PSNR range. We extend the BD measure for storage and transmission rate by projecting S-R-D curves to R-D and S-D planes and we name them BD-R and BD-S respectively. The BD-S represents the average reduction/increase in the amount of data stored on the server for the same PSNR range omitting the transmission rate. BD-R is equivalent to classical BD-R and represents the average bit rate saving/increase for the same PSNR which is transmitted to each user and storage is not taken into account. To evaluate different methods, the pair (BD-R, BD-S) must be considered jointly.

%In most papers, the focus is on the transmission rate and distortion, while the storage requirement is not tackled. This evaluation is natural in  \cite{7328056} since the whole 360-degree content is sent. Therefore, the transmission rate is equal to the storage. By contrast, user-dependent transmission distinguishes Rate and Storage. Thus there is a need to adapt the evaluation. 
It is worth noting that in \cite{8296518}, the BD-R is computed and the sum of storage over all stored qualities are compared. However the sum of stored qualities may not cover the same range of distortion, which leads to an unfair comparison. Introducing BD-S solves this issue because it considers the same range of PSNR for both methods.
 
Two problems can happen with this metric. The first one is due to the fact that sometimes it is not clear how to compare between pairs. For instance, assume (-20\%, 10\%) and (15\%, -10\%) for (BD-R, BD-S) pair between 2 methods (negative values represent percentage saving w.r.t. the reference). Here the former performs better on average in terms of transmission rate and the latter consumes less space on the server for the same PSNR. This problem will be tackled in \cref{subsec:weighted_bd}. Second problem is that BD represents the average performance, but sometimes there are some constraints that the scheme must satisfy. Therefore, we propose iso points in the next subsection to evaluate methods not based on their average behavior, but rather on their performance under some constraint.}


%By projecting S-R-D curves to R-D and S-D planes one can use the Bjontegaard-Delta (BD) measurement \cite{bjontegaard2001calculation} for the storage (BD-S) and transmission rate (BD-R), which correspond to the average rate difference for the same PSNR in storage and transmission rate respectively. This distinction in BD measure for storage and transmission rate is almost overlooked till now. In \cite{8296518} only the BD-R is considered. In \cite{7328056} since the whole 360-degree content is sent, the presented BD-R is actually equivalent to our BD-S measure.

\begin{figure*}[t!]
    \centering
\subfloat[]{%
\fontsize{8pt}{10pt}\selectfont%
\def\svgwidth{0.24\linewidth}%
\input{./figures/iso_distortion_example.eps_tex}%
\label{fig:naive_iso_distortion_curve}}
\hfill
\subfloat[]{%
\fontsize{8pt}{10pt}\selectfont%
\def\svgwidth{0.24\linewidth}%
\input{./figures/iso_distortion_lambda.eps_tex}%
\label{fig:lambda_S_plus_R}}
\hfill
\subfloat[]{%
\fontsize{8pt}{10pt}\selectfont%
\def\svgwidth{0.24\linewidth}%
\input{./figures/iso_distortion_lambda_1_example.eps_tex}%
\label{subfig:iso_distortion_lambda_1}}
\hfill
\subfloat[]{%
\fontsize{8pt}{10pt}\selectfont%
\def\svgwidth{0.24\linewidth}%
\input{./figures/iso_distortion_lambda_2_example.eps_tex}%
\label{subfig:iso_distortion_lambda_2}}
\caption{New metric for the analysis of immersive coding schemes. (a) iso distortion points: each point corresponds to the R,S performance of a compression method for a fixed distortion. Therefore, all points have the same distortion. (b) Projection of the SR plane onto the new axis $R+\lambda S$ (in blue). (c) and (d) Projected S-R-D curves for different $\lambda$ where $\lambda_1 < 
\lambda_2$.}
\label{fig:new_metric}
\end{figure*}

\subsection{Iso points} \label{subsec:iso_points}
{\color{blue}In this section, we propose a set of evaluation tools that can be used when the system must satisfy some constraints. For instance, the service might be constrained to serve the clients with a minimum distortion level $d$. To choose and compare the coding schemes, we introduce the iso-distorsion points: 
$$\{(S_i, R_i, D_i) | D_i = d \text{ and } i \text{ = indices of method}\}$$
where linear interpolation of the S-R-D curve is used to compute the isocurve.

Similarly, iso storage (iso transmission rate) values show that at the same storage (transmission rate) what are the distortion-transmission rate (distortion-storage) values. Depending on what are the constraints of the streaming system (distorion or transmission rate or storage), one can plot iso points and compare the methods on iso values domain.

An example of iso distortion values is shown in \cref{fig:naive_iso_distortion_curve}. Comparing method A and B which have iso distortion values, reveals that method A consumes less bandwidth than method B and it needs lower space on the server to store data. Therefore, method A is preferred over method B. Sometimes isocurves do not help to determine which method is better than the other. For instance, in \cref{fig:naive_iso_distortion_curve} method C takes lower space on the server and method D performs better in terms of transmission rate.}
%choose  To make the comparison possible, we plot iso-distortion points in \cref{fig:iso_distortion}.

\subsection{Weighted BD} \label{subsec:weighted_bd}
{\color{blue}To solve the ambiguities occurred with isocurves and (BD-R,BD-S) pairs, there is a need to adjust the tradeoff between rate and storage. This can be done by introducing a weighted combination:
\begin{equation} \label{eq:linear_combination_storage_transmission_lambda}
\mathbb{E}_{\theta}(R_\theta) + \lambda \cdot S
\end{equation} 
where $\lambda$ balances the importance between storage and transmission rate and is determined by industrial constraints (a high value of $\lambda$ means that storage is more important than transmission rate).
With this definition \eqref{eq:linear_combination_storage_transmission_lambda}, a point in the R-S plane is mapped onto a point on the axis depicted in blue in \cref{fig:lambda_S_plus_R}. This mapping also yields  a projection of the 3D S-R-D curve onto the 2D plane defined by the distortion D and the weighted combination \eqref{eq:linear_combination_storage_transmission_lambda}. Examples of such curves are shown in \cref{subfig:iso_distortion_lambda_1}. Then, from  two such curves, a BD measure can be computed. This is called weighted BD. 


The choice of the regularizer parameter $\lambda$ is crucial, and may yield opposite conclusions when comparing compression methods, see \cref{subfig:iso_distortion_lambda_1,subfig:iso_distortion_lambda_2}.  For instance, \eqref{eq:linear_combination_storage_transmission_lambda} can result from
\begin{equation} \label{eq:linear_combination_storage_transmission_alpha_beta}
\alpha \cdot \mathbb{E}_{\theta}(R_\theta) + \beta \cdot S
\end{equation} 
where the regularizers $\alpha, \beta$ can be used to impose another criterion like delay time for each method. For example, if $\beta$ represents the time per byte that it takes to read the data from the hard drive in the server and $\alpha$ represents the inverse of the bandwidth, then \eqref{eq:linear_combination_storage_transmission_alpha_beta} represents the overall delay time which consists of delay time for the server to read data from its hard drive plus the delay time for the data to be received by the users through the network. By performing BD over this new metric we can compare the delay time over the same PSNR values between two methods.}

%It can be seen that in iso distortion plots it is not always possible to say which one is better than the other. For example, in \cref{fig:iso_distortion} if we compare tiles of size 4480x2240 with tiles of size 640x320 for PSNR of 30, we can see that larger tiles are less efficient in terms of transmission rate, but they are efficient in terms of storage. As another example, for the same PSNR of 30 we can see that cube map is better than tile size 1280x640 in terms of storage, but it results in higher transmission rate. 

%This highlights the idea that we need to define a $\lambda$ which gives the importance (regularization) between storage and transmission, i.e. $S+\lambda \mathbb{E}_{\theta}(R_\theta)$. We propose the $\lambda$-Bjontegaard Delta Rate ($\lambda$-BD-rate). The BD-rate \cite{bjontegaard2001calculation} comparing two codec with eachother while using one as a reference. It measures the bitrate reduction while maintaining the same quality. The ($\lambda$-BD-rate) is the extension of BD-rate while bridging a relation between storage and transmission by a regularizer $\lambda$. It is worth noting that $\lambda=\infty$ means that the server only cares about the storage and $\lambda = 0$ means that only transmission rate is important.

